Multi-level Traffic-Responsive Tilt Camera Surveillance through Predictive Correlated Online Learning

In urban traffic management, the primary challenge of dynamically and efficiently monitoring traffic conditions is compounded by the insufficient utilization of thousands of surveillance cameras along the intelligent transportation system. This paper introduces the multi-level Traffic-responsive Tilt Camera surveillance system (TTC-X), a novel framework designed for dynamic and efficient monitoring and management of traffic in urban networks. By leveraging widely deployed pan-tilt-cameras (PTCs), TTC-X overcomes the limitations of a fixed field of view in traditional surveillance systems by providing mobilized and 360-degree coverage. The innovation of TTC-X lies in the integration of advanced machine learning modules, including a detector-predictor-controller structure, with a novel Predictive Correlated Online Learning (PiCOL) methodology and the Spatial-Temporal Graph Predictor (STGP) for real-time traffic estimation and PTC control. The TTC-X is tested and evaluated under three experimental scenarios (e.g., maximum traffic flow capture, dynamic route planning, traffic state estimation) based on a simulation environment calibrated using real-world traffic data in Brooklyn, New York. The experimental results showed that TTC-X captured over 60\% total number of vehicles at the network level, dynamically adjusted its route recommendation in reaction to unexpected full-lane closure events, and reconstructed link-level traffic states with best MAE less than 1.25 vehicle/hour. Demonstrating scalability, cost-efficiency, and adaptability, TTC-X emerges as a powerful solution for urban traffic management in both cyber-physical and real-world environments.

==> author-statement.tex <==
\section{Acknowledgements}
This work was supported by the C2SMARTER, a Tier 1 U.S. Department of Transportation (USDOT) funded University Transportation Center (UTC) led by New York University funded by USDOT. The contents of this paper only reflect the views of the authors who are responsible for the facts and do not represent any official views of any sponsoring organizations or agencies.

\section{Author Contributions}
The authors confirm their contribution to the paper as follows. Conceptualization: Zilin Bian, Tao Li, Fan Zuo; Data curation: Fan Zuo and Haozhe Lei; Formal analysis: Tao Li, Zilin Bian, Haozhe Lei; Methodology: Tao Li, Zilin Bian, Haozhe Lei, Fan Zuo, Ya-Ting Yang; Validation: Tao Li, Zilin Bian, Haozhe Lei; Visualization: Ya-Ting Yang, Fan Zuo, Tao Li, Zilin Bian; Writing - original draft: Tao Li, Zilin Bian, Fan Zuo, Ya-Ting Yang; and Writing - review \& editing: Tao Li, Zilin Bian, Fan Zuo, Kaan Ozbay, Quanyan Zhu, Zhenning Li. All authors reviewed the results and approved the final version of the manuscript.
